WIT: Wikipedia-based Image Text Dataset for Multimodal Multilingual Machine Learning

The milestone improvements brought about by deep representation learning and pre-training techniques have led to large performance gains across downstream NLP, IR and Vision tasks. Multimodal modeling techniques aim to leverage large high-quality visio-linguistic datasets for learning complementary information (across image and text modalities). In this paper, we introduce the Wikipedia-based Image Text (WIT) Dataset (https://github.com/google-research-datasets/wit) to better facilitate multimodal, multilingual learning. WIT is composed of a curated set of 37.6 million entity rich image-text examples with 11.5 million unique images across 108 Wikipedia languages. Its size enables WIT to be used as a pretraining dataset for multimodal models, as we show when applied to downstream tasks such as image-text retrieval. WIT has four main and unique advantages. First, WIT is the largest multimodal dataset by the number of image-text examples by 3x (at the time of writing). Second, WIT is massively multilingual (first of its kind) with coverage over 100+ languages (each of which has at least 12K examples) and provides cross-lingual texts for many images. Third, WIT represents a more diverse set of concepts and real world entities relative to what previous datasets cover. Lastly, WIT provides a very challenging real-world test set, as we empirically illustrate using an image-text retrieval task as an example.

==> 7_notes.tex <==
% This is scratchpad. This is not included by any other paper.

From CC Paper:
Relevant datasets include the ImageNet
dataset (Deng et al., 2009), with over 14 million
images and 1 million bounding-box annotations,
and the MS-COCO dataset (Lin et al., 2014), with
120,000 images and 5-way image-caption annotations

The Conceptual Captions dataset is programmatically created using a Flume (Chambers et al., 2010) pipeline.

Multi30K: Multilingual English-German Image Descriptions
by Desmond Elliott et al

Multi30K is an extension of the Flickr30K dataset (Young et al., 2014) with 31,014 German translations of English descriptions and 155,070 independently collected German descriptions. The translations were collected from professionally contracted translators, whereas the descriptions were collected from untrained crowd workers. The key difference between these corpora is the relationship between the sentences in different languages. In the translated corpus, we know there is a strong correspondence between the sentences in both languages. In the descriptions corpus, we only know that the sentences, regardless of the language, are supposed to describe the same image. 

145,000 training, 5,070 development, and 5,000 test descriptions
% Interesting: Multi30K paper does not have a single experiment.
% it is only about creating the DE dataset.


From RWorld paper:
The success stories of VLP in recent literature involve pre-training approaches using joint image and text as input (Lu et al., 2019; Li et al., 2019;
Chen et al., 2019; Tan and Bansal, 2019; Alberti et al., 2019; Su et al., 2020; Zhou et al., 2020; Li et al., 2020a; Lu et al., 2020), while mainly considering classification- or regression-based tasks: vocab-based/multiple-choice VQA, referring expressions, multi-modal verification, and image-text matching for retrieval. The important finding there is that those tasks benefit from learning fused representations suitable for joint image-and-text understanding.

There is mention of this : Conceptual Captions CC17M We construct this
third dataset ourselves.
% HOW SHOULD WE CITE THIS? (is Rworld public?)
16,913,177 image-text pairs

the Open Images dataset (Kuznetsova et al., 2018; Krasin et al.,
2017) covers one order of magnitude more objects
(600 classes) than COCO (Lin et al., 2014) (80
classes).

% CHECK this out for a good dual encoder explanation - which can be used or
% referenced as needed. (if we want).
End-to-End Retrieval in Continuous Space
Daniel Gillick

From MS-COCO paper:
The Microsoft Common Objects in COntext (MS
COCO) dataset contains 91 common object categories
with 82 of them having more than 5,000 labeled instances, Fig. 6. In total the dataset has 2,500,000 labeled
instances in 328,000 images. In contrast to the popular
ImageNet dataset [1], COCO has fewer categories but
more instances per category.

y, ImageNet [1] made a striking departure from
the incremental increase in dataset sizes. They proposed
the creation of a dataset containing 22k categories with
500-1000 images each
=> Right now ImageNet consists of 14M images.

% table back up - just in case.
\begin{table}
  \caption{Statistics of the final WIT dataset and availability of different fields.}
  \label{tab:wit-dataset-numbers}
  \vspace{-1em}
  \begin{tabular}{|c|c|c|c|c|c|c|}
    \hline 
    \textbf{Type} 
    & \textbf{Image-Text}
    & \textbf{Images}
    & \textbf{Text}
    & \textbf{Ref.}
    & \textbf{Attr.}
    & \textbf{Alt.} \\ 
    \hline 
    \text{Train} 
%    & \text{37,139,639} 
     & \text{37.13M} 
    & 11.4M & 57.1M & 34.8M & 16.9M & 5.3M 
    \\  
    \hline 
    \text{Val} 
%    & \text{261,809} 
    & \text{261.8K} 
    & 58K & 373K & 193K & 150K & 29K
    \\
    \hline 
    \text{Test} 
%    & \text{210,690} 
    & \text{210.7K} 
    & 57K & 334K & 200K & 104K & 29K
    \\
    \hline 
    \textbf{Total} 
%    & \textbf{37,612,138} 
    & \textbf{37.6M} 
    & \textbf{11.5M} & \textbf{57.8M} & \textbf{35.2M} & \textbf{17.2M} & \textbf{5.3M}
    \\
  \hline
\end{tabular}
\vspace{-1.5em}
\end{table}


\begin{table}
  \caption{WIT: Human Evaluation : Language Split}
  \label{tab:wit-he-lang-split}
  \begin{tabular}{|c|c|c|}
    \hline 
    \textbf{Language} 
    & \textbf{Num. Examples}
    & \textbf{Percent} \\ 
  \hline
    Total EN & 2793 & 63.58\% \\
  \hline
    Total DE & 300 & 6.83\% \\ 
  \hline
    Total ES & 300 & 6.83\% \\
  \hline
    Total FR & 300 & 6.83\% \\
  \hline
    Total HI & 100 & 2.28\% \\
  \hline
    Total RU & 300 & 6.83\% \\
  \hline
    Total ZH & 300 & 6.83\% \\
  \hline
    \textbf{Total} & \textbf{4393} & \textbf{100\%} \\
    \hline
\end{tabular}
\end{table}
% Total Ratings 	39537


% This was in Section 4.
\subsection{Experiment 2: Effectiveness of Various Text Fields}

WIT has over 37 million image-text sets. Unlike other datasets, each image has a variety of text captions that it can be associated with. The reference description (the caption right in the context of the Wikipedia page) and the attribution description (the caption on the image's dedicated Wikimedia page) are the two popular relevant choices. However, there are a few other text sources that can be utilized. For e.g., the field called image caption (which is an additional in the image asset page), the Wikipedia page title, the section title (either by itself or as a hierarchical title), the Wikipedia's page description (which tends to be general as it relates to the whole page) and the Section text (which is more specific to the image since this is the text of the section in which the image appears). Our second set of experiments was to use various text as the choice for the text encoder and evaluated its zero-shot performance on the various WIT test sets. In addition to using the WIT test as a whole, we also split the test set into two : English only and I18N only (all languages except English). The results are shown in table \ref{tab:wit-de-exp-retrieval-2}. The concatenation of reference description and attribution description gave the best performance.

%%%%
%%%% TABLE 2 : e41, e42, e43, e26 : WIT (all / en / i18n): r1/r5
%%%%
\begin{table}[]
\caption{Dual Encoder Model : Zero-shot Evaluation on WIT test set (all, en, i18n) of various Text Fields for a Retrieval Task}
\label{tab:wit-de-exp-retrieval-2}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{Exp}} & \multirow{2}{*}{\textbf{Text}} & \multicolumn{2}{c|}{\textbf{WIT-All}} & \multicolumn{2}{c|}{\textbf{WIT-EN}} & \multicolumn{2}{c|}{\textbf{WIT-I18N}} \\ \cline{3-8}
    & & \textbf{R@1} & \textbf{R@5} & \textbf{R@1} & \textbf{R@5} & \textbf{R@1} & \textbf{R@5}  \\ \hline
%
% & \textbf{e41}     % Exp.
\textbf{WIT}     % Pretrain
& \textbf{ref}     % Text Field
& \text{0.126}     % W-ALL R@1
& \text{0.258}     % W-ALL R@5
& \text{0.169}     % W-EN R@1
& \text{0.358}     % W-EN R@5
& \text{0.114}     % W-I18N R@1
& \text{0.236} \\ \hline
% & \textbf{e42}     % Exp.
\textbf{WIT}     % Pretrain
& \textbf{attr}     % Text Field
& \text{0.293}     % W-ALL R@1
& \text{0.55}     % W-ALL R@5
& \text{0.272}     % W-EN R@1
& \text{0.523}     % W-EN R@5
& \text{0.293}     % W-I18N R@1
& \text{0.523} \\ \hline
% & \textbf{e43}     % Exp.
\textbf{WIT}     % Pretrain
& \textbf{ref+attr}     % Text Field
& \textbf{0.346}     % W-ALL R@1
& \textbf{0.642}     % W-ALL R@5
& \textbf{0.344}     % W-EN R@1
& \textbf{0.64}     % W-EN R@5
& \textbf{0.344}     % W-I18N R@1
& \textbf{0.633} \\ \hline
% & \textbf{e26}     % Exp.
\textbf{CC}     % Pretrain
& \textbf{text}     % Text Field
& \text{0.048}     % W-ALL R@1
& \text{0.122}     % W-ALL R@5
& \text{0.072}     % W-EN R@1
& \text{0.186}     % W-EN R@5
& \text{0.041}     % W-I18N R@1
& \text{0.11} \\ \hline
\end{tabular}
\end{table}


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> REF_4c_exp_full_table.tex <==
% This table/file is not used directly since this table is very big.
% But this has all the data.

\begin{table}
  \caption{Dual Encoder Model: Image-Text Retrieval}
  \label{tab:wit-de-retrieval}
  \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
& \textbf{Exp.}
& \textbf{Pretrain}
& \textbf{Text Field}
& \textbf{Finetune}
& \textbf{COCO  R@1}
& \textbf{COCO  R@3}
& \textbf{COCO  R@5}
& \textbf{F-30K  R@1}
& \textbf{F-30K  R@3}
& \textbf{F-30K  R@5}
& \textbf{W-ALL R@1}
& \textbf{W-ALL R@3}
& \textbf{W-ALL R@5}
& \textbf{W-EN R@1}
& \textbf{W-EN R@3}
& \textbf{W-EN R@5}
& \textbf{W-I18N R@1}
& \textbf{W-I18N R@3}
& \textbf{W-I18N R@5}
& \textbf{W-CS R@1}
& \textbf{W-CS R@3}
& \textbf{W-CS R@5}
& \textbf{M-CS R@1}
& \textbf{M-CS R@3}
& \textbf{M-CS R@5}
& \textbf{W-DE R@1}
& \textbf{W-DE R@3}
& \textbf{W-DE R@5}
& \textbf{M-DE R@1}
& \textbf{M-DE R@3}
& \textbf{M-DE R@5}
& \textbf{W-FR R@1}
& \textbf{W-FR R@3}
& \textbf{W-FR R@5}
& \textbf{M-FR R@1}
& \textbf{M-FR R@3}
& \textbf{M-FR R@5}\\
\hline
& \textbf{e27}     % Exp.
& \textbf{WIT-EN}     % Pretrain
& \textbf{page_title}     % Text Field
& \textbf{}     % Finetune
& \textbf{0.018}     % COCO  R@1
& \textbf{0.043}     % COCO  R@3
& \textbf{0.064}     % COCO  R@5
& \textbf{0.011}     % F-30K  R@1
& \textbf{0.027}     % F-30K  R@3
& \textbf{0.04}     % F-30K  R@5
& \textbf{0.067}     % W-ALL R@1
& \textbf{0.122}     % W-ALL R@3
& \textbf{0.152}     % W-ALL R@5
& \textbf{0.161}     % W-EN R@1
& \textbf{0.294}     % W-EN R@3
& \textbf{0.369}     % W-EN R@5
& \textbf{0.044}     % W-I18N R@1
& \textbf{0.082}     % W-I18N R@3
& \textbf{0.106}     % W-I18N R@5
& \textbf{0.04}     % W-CS R@1
& \textbf{0.08}     % W-CS R@3
& \textbf{0.102}     % W-CS R@5
& \textbf{}     % M-CS R@1
& \textbf{}     % M-CS R@3
& \textbf{}     % M-CS R@5
& \textbf{0.046}     % W-DE R@1
& \textbf{0.086}     % W-DE R@3
& \textbf{0.11}     % W-DE R@5
& \textbf{}     % M-DE R@1
& \textbf{}     % M-DE R@3
& \textbf{}     % M-DE R@5
& \textbf{0.054}     % W-FR R@1
& \textbf{0.105}     % W-FR R@3
& \textbf{0.136}     % W-FR R@5
& \textbf{}     % M-FR R@1
& \textbf{}     % M-FR R@3
& \textbf{}     % M-FR R@5\\
\hline
& \textbf{e28}     % Exp.
& \textbf{CC}     % Pretrain
& \textbf{raw_text}     % Text Field
& \textbf{}     % Finetune
& \textbf{0.147}     % COCO  R@1
& \textbf{0.299}     % COCO  R@3
& \textbf{0.392}     % COCO  R@5
& \textbf{0.109}     % F-30K  R@1
& \textbf{0.237}     % F-30K  R@3
& \textbf{0.321}     % F-30K  R@5
& \textbf{0.012}     % W-ALL R@1
& \textbf{0.024}     % W-ALL R@3
& \textbf{0.032}     % W-ALL R@5
& \textbf{0.028}     % W-EN R@1
& \textbf{0.058}     % W-EN R@3
& \textbf{0.078}     % W-EN R@5
& \textbf{0.007}     % W-I18N R@1
& \textbf{0.015}     % W-I18N R@3
& \textbf{0.021}     % W-I18N R@5
& \textbf{0.006}     % W-CS R@1
& \textbf{0.013}     % W-CS R@3
& \textbf{0.018}     % W-CS R@5
& \textbf{}     % M-CS R@1
& \textbf{}     % M-CS R@3
& \textbf{}     % M-CS R@5
& \textbf{0.007}     % W-DE R@1
& \textbf{0.017}     % W-DE R@3
& \textbf{0.025}     % W-DE R@5
& \textbf{}     % M-DE R@1
& \textbf{}     % M-DE R@3
& \textbf{}     % M-DE R@5
& \textbf{0.009}     % W-FR R@1
& \textbf{0.02}     % W-FR R@3
& \textbf{0.028}     % W-FR R@5
& \textbf{}     % M-FR R@1
& \textbf{}     % M-FR R@3
& \textbf{}     % M-FR R@5\\
\hline
& \textbf{e34a}     % Exp.
& \textbf{WIT-ALL}     % Pretrain
& \textbf{page_title}     % Text Field
& \textbf{WIT-ALL}     % Finetune
& \textbf{0.069}     % COCO  R@1
& \textbf{0.156}     % COCO  R@3
& \textbf{0.217}     % COCO  R@5
& \textbf{0.047}     % F-30K  R@1
& \textbf{0.11}     % F-30K  R@3
& \textbf{0.155}     % F-30K  R@5
& \textbf{0.1}     % W-ALL R@1
& \textbf{0.174}     % W-ALL R@3
& \textbf{0.214}     % W-ALL R@5
& \textbf{0.199}     % W-EN R@1
& \textbf{0.339}     % W-EN R@3
& \textbf{0.412}     % W-EN R@5
& \textbf{0.078}     % W-I18N R@1
& \textbf{0.143}     % W-I18N R@3
& \textbf{0.18}     % W-I18N R@5
& \textbf{0.065}     % W-CS R@1
& \textbf{0.127}     % W-CS R@3
& \textbf{0.164}     % W-CS R@5
& \textbf{0.001}     % M-CS R@1
& \textbf{0.003}     % M-CS R@3
& \textbf{0.005}     % M-CS R@5
& \textbf{0.078}     % W-DE R@1
& \textbf{0.145}     % W-DE R@3
& \textbf{0.186}     % W-DE R@5
& \textbf{0.001}     % M-DE R@1
& \textbf{0.003}     % M-DE R@3
& \textbf{0.006}     % M-DE R@5
& \textbf{0.086}     % W-FR R@1
& \textbf{0.16}     % W-FR R@3
& \textbf{0.203}     % W-FR R@5
& \textbf{0.001}     % M-FR R@1
& \textbf{0.003}     % M-FR R@3
& \textbf{0.005}     % M-FR R@5\\
\hline
& \textbf{e35a}     % Exp.
& \textbf{CC}     % Pretrain
& \textbf{page_title}     % Text Field
& \textbf{CC}     % Finetune
& \textbf{0.126}     % COCO  R@1
& \textbf{0.259}     % COCO  R@3
& \textbf{0.346}     % COCO  R@5
& \textbf{0.095}     % F-30K  R@1
& \textbf{0.202}     % F-30K  R@3
& \textbf{0.268}     % F-30K  R@5
& \textbf{0.01}     % W-ALL R@1
& \textbf{0.021}     % W-ALL R@3
& \textbf{0.029}     % W-ALL R@5
& \textbf{0.024}     % W-EN R@1
& \textbf{0.051}     % W-EN R@3
& \textbf{0.068}     % W-EN R@5
& \textbf{0.006}     % W-I18N R@1
& \textbf{0.014}     % W-I18N R@3
& \textbf{0.019}     % W-I18N R@5
& \textbf{0.006}     % W-CS R@1
& \textbf{0.014}     % W-CS R@3
& \textbf{0.019}     % W-CS R@5
& \textbf{0.001}     % M-CS R@1
& \textbf{0.003}     % M-CS R@3
& \textbf{0.005}     % M-CS R@5
& \textbf{0.007}     % W-DE R@1
& \textbf{0.016}     % W-DE R@3
& \textbf{0.022}     % W-DE R@5
& \textbf{0.001}     % M-DE R@1
& \textbf{0.003}     % M-DE R@3
& \textbf{0.006}     % M-DE R@5
& \textbf{0.008}     % W-FR R@1
& \textbf{0.018}     % W-FR R@3
& \textbf{0.025}     % W-FR R@5
& \textbf{0.001}     % M-FR R@1
& \textbf{0.003}     % M-FR R@3
& \textbf{0.005}     % M-FR R@5\\
\hline
& \textbf{e36}     % Exp.
& \textbf{WIT-ALL}     % Pretrain
& \textbf{ref_attr}     % Text Field
& \textbf{Flickr30K}     % Finetune
& \textbf{0.128}     % COCO  R@1
& \textbf{0.268}     % COCO  R@3
& \textbf{0.358}     % COCO  R@5
& \textbf{0.163}     % F-30K  R@1
& \textbf{0.359}     % F-30K  R@3
& \textbf{0.458}     % F-30K  R@5
& \textbf{0.291}     % W-ALL R@1
& \textbf{0.489}     % W-ALL R@3
& \textbf{0.572}     % W-ALL R@5
& \textbf{0.276}     % W-EN R@1
& \textbf{0.476}     % W-EN R@3
& \textbf{0.57}     % W-EN R@5
& \textbf{0.287}     % W-I18N R@1
& \textbf{0.473}     % W-I18N R@3
& \textbf{0.567}     % W-I18N R@5
& \textbf{0/214}     % W-CS R@1
& \textbf{0.401}     % W-CS R@3
& \textbf{0/492}     % W-CS R@5
& \textbf{0.001}     % M-CS R@1
& \textbf{0.003}     % M-CS R@3
& \textbf{0.005}     % M-CS R@5
& \textbf{0.236}     % W-DE R@1
& \textbf{0.411}     % W-DE R@3
& \textbf{0.508}     % W-DE R@5
& \textbf{0.001}     % M-DE R@1
& \textbf{0.003}     % M-DE R@3
& \textbf{0.005}     % M-DE R@5
& \textbf{0.257}     % W-FR R@1
& \textbf{0.445}     % W-FR R@3
& \textbf{0.508}     % W-FR R@5
& \textbf{0.001}     % M-FR R@1
& \textbf{0.003}     % M-FR R@3
& \textbf{0.006}     % M-FR R@5\\
\hline
& \textbf{e37}     % Exp.
& \textbf{CC}     % Pretrain
& \textbf{ref_attr}     % Text Field
& \textbf{Flickr30K}     % Finetune
& \textbf{0.188}     % COCO  R@1
& \textbf{0.365}     % COCO  R@3
& \textbf{0.466}     % COCO  R@5
& \textbf{0.201}     % F-30K  R@1
& \textbf{0.394}     % F-30K  R@3
& \textbf{0.497}     % F-30K  R@5
& \textbf{0.047}     % W-ALL R@1
& \textbf{0.09}     % W-ALL R@3
& \textbf{0.115}     % W-ALL R@5
& \textbf{0.068}     % W-EN R@1
& \textbf{0.134}     % W-EN R@3
& \textbf{0.176}     % W-EN R@5
& \textbf{0.04}     % W-I18N R@1
& \textbf{0.078}     % W-I18N R@3
& \textbf{0.104}     % W-I18N R@5
& \textbf{0/032}     % W-CS R@1
& \textbf{0.067}     % W-CS R@3
& \textbf{0.088}     % W-CS R@5
& \textbf{0.001}     % M-CS R@1
& \textbf{0.003}     % M-CS R@3
& \textbf{0.005}     % M-CS R@5
& \textbf{0.028}     % W-DE R@1
& \textbf{0.055}     % W-DE R@3
& \textbf{0.072}     % W-DE R@5
& \textbf{0.001}     % M-DE R@1
& \textbf{0.003}     % M-DE R@3
& \textbf{0.005}     % M-DE R@5
& \textbf{0.036}     % W-FR R@1
& \textbf{0.073}     % W-FR R@3
& \textbf{0.094}     % W-FR R@5
& \textbf{0.001}     % M-FR R@1
& \textbf{0.003}     % M-FR R@3
& \textbf{0.006}     % M-FR R@5\\
\hline
& \textbf{e41}     % Exp.
& \textbf{WIT-ALL}     % Pretrain
& \textbf{ref}     % Text Field
& \textbf{}     % Finetune
& \textbf{0.034}     % COCO  R@1
& \textbf{0.082}     % COCO  R@3
& \textbf{0.119}     % COCO  R@5
& \textbf{0.022}     % F-30K  R@1
& \textbf{0.055}     % F-30K  R@3
& \textbf{0.085}     % F-30K  R@5
& \textbf{0.126}     % W-ALL R@1
& \textbf{0.212}     % W-ALL R@3
& \textbf{0.258}     % W-ALL R@5
& \textbf{0.169}     % W-EN R@1
& \textbf{0.295}     % W-EN R@3
& \textbf{0.358}     % W-EN R@5
& \textbf{0.114}     % W-I18N R@1
& \textbf{0.195}     % W-I18N R@3
& \textbf{0.236}     % W-I18N R@5
& \textbf{0.096}     % W-CS R@1
& \textbf{0.186}     % W-CS R@3
& \textbf{0.234}     % W-CS R@5
& \textbf{0.001}     % M-CS R@1
& \textbf{0.002}     % M-CS R@3
& \textbf{0.005}     % M-CS R@5
& \textbf{0.117}     % W-DE R@1
& \textbf{0.203}     % W-DE R@3
& \textbf{0.254}     % W-DE R@5
& \textbf{0.001}     % M-DE R@1
& \textbf{0.003}     % M-DE R@3
& \textbf{0.005}     % M-DE R@5
& \textbf{0.116}     % W-FR R@1
& \textbf{0.201}     % W-FR R@3
& \textbf{0.242}     % W-FR R@5
& \textbf{0.001}     % M-FR R@1
& \textbf{0.003}     % M-FR R@3
& \textbf{0.004}     % M-FR R@5\\
\hline
& \textbf{e42}     % Exp.
& \textbf{WIT-ALL}     % Pretrain
& \textbf{attr}     % Text Field
& \textbf{}     % Finetune
& \textbf{0.058}     % COCO  R@1
& \textbf{0.132}     % COCO  R@3
& \textbf{0.185}     % COCO  R@5
& \textbf{0.04}     % F-30K  R@1
& \textbf{0.093}     % F-30K  R@3
& \textbf{0.133}     % F-30K  R@5
& \textbf{0.293}     % W-ALL R@1
& \textbf{0.472}     % W-ALL R@3
& \textbf{0.55}     % W-ALL R@5
& \textbf{0.272}     % W-EN R@1
& \textbf{0.445}     % W-EN R@3
& \textbf{0.523}     % W-EN R@5
& \textbf{0.293}     % W-I18N R@1
& \textbf{0.475}     % W-I18N R@3
& \textbf{0.523}     % W-I18N R@5
& \textbf{0.216}     % W-CS R@1
& \textbf{0.39}     % W-CS R@3
& \textbf{0.473}     % W-CS R@5
& \textbf{0.001}     % M-CS R@1
& \textbf{0.002}     % M-CS R@3
& \textbf{0.005}     % M-CS R@5
& \textbf{0.244}     % W-DE R@1
& \textbf{0.408}     % W-DE R@3
& \textbf{0.486}     % W-DE R@5
& \textbf{0.001}     % M-DE R@1
& \textbf{0.003}     % M-DE R@3
& \textbf{0.005}     % M-DE R@5
& \textbf{0.262}     % W-FR R@1
& \textbf{0.435}     % W-FR R@3
& \textbf{0.513}     % W-FR R@5
& \textbf{0.001}     % M-FR R@1
& \textbf{0.003}     % M-FR R@3
& \textbf{0.004}     % M-FR R@5\\
\hline
& \textbf{e43}     % Exp.
& \textbf{WIT-ALL}     % Pretrain
& \textbf{ref_attr}     % Text Field
& \textbf{}     % Finetune
& \textbf{0.074}     % COCO  R@1
& \textbf{0.166}     % COCO  R@3
& \textbf{0.228}     % COCO  R@5
& \textbf{0.054}     % F-30K  R@1
& \textbf{0.119}     % F-30K  R@3
& \textbf{0.165}     % F-30K  R@5
& \textbf{0.346}     % W-ALL R@1
& \textbf{0.554}     % W-ALL R@3
& \textbf{0.642}     % W-ALL R@5
& \textbf{0.344}     % W-EN R@1
& \textbf{0.551}     % W-EN R@3
& \textbf{0.64}     % W-EN R@5
& \textbf{0.344}     % W-I18N R@1
& \textbf{0.546}     % W-I18N R@3
& \textbf{0.633}     % W-I18N R@5
& \textbf{0.253}     % W-CS R@1
& \textbf{0.46}     % W-CS R@3
& \textbf{0.553}     % W-CS R@5
& \textbf{0.001}     % M-CS R@1
& \textbf{0.004}     % M-CS R@3
& \textbf{0.006}     % M-CS R@5
& \textbf{0.286}     % W-DE R@1
& \textbf{0.473}     % W-DE R@3
& \textbf{0.562}     % W-DE R@5
& \textbf{0.001}     % M-DE R@1
& \textbf{0.003}     % M-DE R@3
& \textbf{0.005}     % M-DE R@5
& \textbf{0.312}     % W-FR R@1
& \textbf{0.514}     % W-FR R@3
& \textbf{0.599}     % W-FR R@5
& \textbf{0.001}     % M-FR R@1
& \textbf{0.003}     % M-FR R@3
& \textbf{0.006}     % M-FR R@5\\
\hline
& \textbf{e26}     % Exp.
& \textbf{CC}     % Pretrain
& \textbf{raw_text}     % Text Field
& \textbf{}     % Finetune
& \textbf{0.145}     % COCO  R@1
& \textbf{0.294}     % COCO  R@3
& \textbf{0.385}     % COCO  R@5
& \textbf{0.111}     % F-30K  R@1
& \textbf{0.241}     % F-30K  R@3
& \textbf{0.32}     % F-30K  R@5
& \textbf{0.048}     % W-ALL R@1
& \textbf{0.095}     % W-ALL R@3
& \textbf{0.122}     % W-ALL R@5
& \textbf{0.072}     % W-EN R@1
& \textbf{0.146}     % W-EN R@3
& \textbf{0.186}     % W-EN R@5
& \textbf{0.041}     % W-I18N R@1
& \textbf{0.083}     % W-I18N R@3
& \textbf{0.11}     % W-I18N R@5
& \textbf{0.032}     % W-CS R@1
& \textbf{0.074}     % W-CS R@3
& \textbf{0.096}     % W-CS R@5
& \textbf{0.0005}     % M-CS R@1
& \textbf{0.002}     % M-CS R@3
& \textbf{0.004}     % M-CS R@5
& \textbf{0.032}     % W-DE R@1
& \textbf{0.063}     % W-DE R@3
& \textbf{0.084}     % W-DE R@5
& \textbf{0.001}     % M-DE R@1
& \textbf{0.003}     % M-DE R@3
& \textbf{0.005}     % M-DE R@5
& \textbf{0.04}     % W-FR R@1
& \textbf{0.078}     % W-FR R@3
& \textbf{0.104}     % W-FR R@5
& \textbf{0.001}     % M-FR R@1
& \textbf{0.002}     % M-FR R@3
& \textbf{0.004}     % M-FR R@5\\
\hline

\end{tabular}
\end{table}


%%
%% THIS IS THE OLD EXPERIMENTS TABLE
%%

\begin{table}[]
\caption{Dual Encoder Model with Retrieval Task}
\label{tab:wit-de-exp-retrieval}
\begin{tabular}{|c|c|c|c|}
\hline
\multirow{2}{*}{Text} & \multicolumn{3}{c|}{Recall@1} \\ \cline{2-4} 
                  & Flickr30K & MS-COCO & WIT \\ \hline
  \text{attr + page}
    & \text{0.045}
    & \text{0.033}
    & \text{0.289}\\
    \hline
    \text{attr + title}
    & \text{0.053}
    & \text{0.033}
    & \text{0.255}\\
    \hline
    \text{ref + page}
    & \text{0.043}
    & \text{0.031}
    & \text{0.266}\\
    \hline
    \text{ref + title}
    & \text{0.05}
    & \text{0.041}
    & \text{0.217}\\
    \hline
    \text{attr (len20)}
    & \text{0.05}
    & \text{0.034}
    & \text{0.234}\\
    \hline
    \text{attr (len 40)}
    & \text{0.042}
    & \text{0.027}
    & \text{0.221}\\
    \hline
    \text{ref (len20)}
    & \text{0.04}
    & \text{0.033}
    & \text{0.175}\\
    \hline
    \text{ref (len 40)}
    & \text{0.032}
    & \text{0.025}
    & \text{0.142}\\
    \hline
    \text{ref + attr (len 20)}
    & \text{0.06}
    & \text{0.042}
    & \text{0.263}\\
  \hline
\end{tabular}
\end{table}


% MODEL TABLE
% Use this as a starting point for new tables.
\begin{table}[]
\caption{Dual Encoder Model : Retrieval Task}
\label{tab:wit-de-exp-retrieval-1}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Text} & \multicolumn{3}{c|}{Set1} & \multicolumn{3}{c|}{Set2} & \multicolumn{3}{c|}{Set3} \\ \cline{2-10}
      & R@1 & R@3 & R@5 & R@1 & R@3 & R@5 & R@1 & R@3 & R@5  \\ \hline
Exp 1 & 0.045 & 0.033 & 0.289 & 0.045 & 0.033 & 0.289 & 0.045 & 0.033 & 0.289 \\ \hline
% there should be 1 text field followed by 9 exp values. 
\end{tabular}
\end{table}

% The above table has 10 columns and that does not fit well - so creating
% this table with 7 columns. (Skipping R@3).
\begin{table}[]
\caption{Dual Encoder Model : Retrieval Task}
\label{tab:wit-de-exp-retrieval-1}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Text} & \multicolumn{3}{c|}{Set1} & \multicolumn{3}{c|}{Set2} & \multicolumn{3}{c|}{Set3} \\ \cline{2-7}
     & R@1 & R@5 & R@1 & R@5 & R@1 & R@5  \\ \hline
Exp 1 & 0.045 & 0.289 & 0.045 & 0.289 & 0.045 & 0.289 \\ \hline
% there should be 1 text field followed by 9 exp values. 
\end{tabular}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%
%%%%
%%%% TABLE 1 : e43, e26 : COCO / Flickr / WIT : r1/r5
%%%%
\begin{table}[]
\caption{Dual Encoder Model : Zero-shot comparison on Flickr30K, COCO and WIT test set for a Retrieval Task}
\label{tab:wit-de-exp-retrieval-1}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Exp} & \multicolumn{2}{c|}{MS-COCO} & \multicolumn{2}{c|}{Flickr30K} & \multicolumn{2}{c|}{WIT-Test} \\ \cline{2-7}
    & R@1 & R@5 & R@1 & R@5 & R@1 & R@5  \\ \hline
%
% there should be 1 text field followed by 6 exp values. 
% Exp 1 & 0.045 & 0.289 & 0.045 & 0.289 & 0.045 & 0.289 \\ \hline
%
% & \textbf{e43}     % Exp.
\textbf{WIT-ALL}     % Pretrain
& \textbf{0.074}     % COCO  R@1
& \textbf{0.228}     % COCO  R@5
& \textbf{0.054}     % F-30K  R@1
& \textbf{0.165}     % F-30K  R@5
& \textbf{0.346}     % W-ALL R@1
& \textbf{0.642}\\  \hline
% & \textbf{e26}     % Exp.
\textbf{CC}     % Pretrain
& \textbf{0.145}     % COCO  R@1
& \textbf{0.385}     % COCO  R@5
& \textbf{0.111}     % F-30K  R@1
& \textbf{0.32}     % F-30K  R@5
& \textbf{0.048}     % W-ALL R@1
& \textbf{0.122}\\   \hline
\end{tabular}
\end{table}

%%%%
%%%% TABLE 2 : e41, e42, e43, e26 : WIT (all / en / i18n): r1/r5
%%%%
\begin{table}[]
\caption{Dual Encoder Model : Zero-shot comparison on WIT test set (all, en, i18n) for a Retrieval Task}
\label{tab:wit-de-exp-retrieval-2}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Exp} & \multicolumn{2}{c|}{WIT-All} & \multicolumn{2}{c|}{WIT-EN} & \multicolumn{2}{c|}{WIT-I18N} \\ \cline{2-7}
    & R@1 & R@5 & R@1 & R@5 & R@1 & R@5  \\ \hline
%
% & \textbf{e41}     % Exp.
\textbf{WIT (ref)}     % Pretrain
% & \textbf{ref}     % Text Field
& \textbf{0.126}     % W-ALL R@1
& \textbf{0.258}     % W-ALL R@5
& \textbf{0.169}     % W-EN R@1
& \textbf{0.358}     % W-EN R@5
& \textbf{0.114}     % W-I18N R@1
& \textbf{0.236} \\ \hline
% & \textbf{e42}     % Exp.
\textbf{WIT (attr)}     % Pretrain
% & \textbf{attr}     % Text Field
& \textbf{0.293}     % W-ALL R@1
& \textbf{0.55}     % W-ALL R@5
& \textbf{0.272}     % W-EN R@1
& \textbf{0.523}     % W-EN R@5
& \textbf{0.293}     % W-I18N R@1
& \textbf{0.523} \\ \hline
% & \textbf{e43}     % Exp.
\textbf{WIT (ref+attr)}     % Pretrain
% & \textbf{ref_attr}     % Text Field
& \textbf{0.346}     % W-ALL R@1
& \textbf{0.642}     % W-ALL R@5
& \textbf{0.344}     % W-EN R@1
& \textbf{0.64}     % W-EN R@5
& \textbf{0.344}     % W-I18N R@1
& \textbf{0.633} \\ \hline
% & \textbf{e26}     % Exp.
\textbf{CC}     % Pretrain
% & \textbf{raw_text}     % Text Field
& \textbf{0.048}     % W-ALL R@1
& \textbf{0.122}     % W-ALL R@5
& \textbf{0.072}     % W-EN R@1
& \textbf{0.186}     % W-EN R@5
& \textbf{0.041}     % W-I18N R@1
& \textbf{0.11} \\ \hline
\end{tabular}
\end{table}


%%%%
%%%% TABLE 3 : e43, e26 : W-CS, W-DE, W-FR, M-CS, M-DE, M-FR : r5
%%%%
\begin{table}[]
\caption{Dual Encoder Model : Zero-shot comparison on Multi30K and WIT test sets (CS, DE, FR) for a Retrieval Task}
\label{tab:wit-de-exp-retrieval-3}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Exp} & \multicolumn{3}{c|}{Multi30K-R@5} & \multicolumn{3}{c|}{WIT-R@5} \\ \cline{2-7}
    & CS & DE & FR & CS & DE & FR  \\ \hline
%
% & \textbf{e43}     % Exp.
\textbf{WIT-ALL}     % Pretrain
% & \textbf{ref_attr}     % Text Field
& \textbf{0.006}     % M-CS R@5
& \textbf{0.005}     % M-DE R@5
& \textbf{0.006}     % M-FR R@5
& \textbf{0.553}     % W-CS R@5
& \textbf{0.562}     % W-DE R@5
& \textbf{0.599} \\ \hline
% & \textbf{e26}     % Exp.
\textbf{CC}     % Pretrain
% & \textbf{raw_text}     % Text Field
& \textbf{0.004}     % M-CS R@5
& \textbf{0.005}     % M-DE R@5
& \textbf{0.004}     % M-FR R@5
& \textbf{0.096}     % W-CS R@5
& \textbf{0.084}     % W-DE R@5
& \textbf{0.104} \\ \hline

\end{tabular}
\end{table}


%%%%
%%%% TABLE 4 : e27, e28, e34a, e35a : page_title : w-all, en, i18n : r1/r5
%%%%
\begin{table}[]
\caption{Dual Encoder Model : Zero-shot and Finetuned comparison on WIT (image, title) test set for a Retrieval Task}
\label{tab:wit-de-exp-retrieval-4}
\begin{tabular}{|c|c|c|c|}
\hline
\multirow{2}{*}{Exp} & \multicolumn{3}{c|}{WIT-All}  \\ \cline{2-4}
                      & R@1 & R@3 & R@5  \\ \hline
%
% & \textbf{e27}     % Exp.
\textbf{WIT-EN (None)}     % Pretrain
% & \textbf{page_title}     % Text Field
% & \textbf{None}     % Finetune
& \textbf{0.067}     % W-ALL R@1
& \textbf{0.122}     % W-ALL R@3
& \textbf{0.152} \\ \hline
% & \textbf{e28}     % Exp.
\textbf{CC (None)}     % Pretrain
% & \textbf{raw_text}     % Text Field
% & \textbf{None}     % Finetune
& \textbf{0.012}     % W-ALL R@1
& \textbf{0.024}     % W-ALL R@3
& \textbf{0.032} \\ \hline
% & \textbf{e34a}     % Exp.
\textbf{WIT-ALL (WIT-ALL)}     % Pretrain
% & \textbf{page_title}     % Text Field
% & \textbf{WIT-ALL}     % Finetune
& \textbf{0.1}     % W-ALL R@1
& \textbf{0.174}     % W-ALL R@3
& \textbf{0.214} \\ \hline
% & \textbf{e35a}     % Exp.
\textbf{CC (CC)}     % Pretrain
% & \textbf{page_title}     % Text Field
% & \textbf{CC}     % Finetune
& \textbf{0.01}     % W-ALL R@1
& \textbf{0.021}     % W-ALL R@3
& \textbf{0.029} \\ \hline
\end{tabular}
\end{table}





==> REF_Old_4_experiments.tex <==
\section{Multimodal Experiments}


\ks{This is the version as of Dec 20. I am updating with all the new experiments in 4a\_experiments.tex.}

We conducted a few different variations of popular models using WIT as a pretraining dataset. Primarily, the main architecture of focus was a dual-encoder model with a text encoder (text tower) and an image encoder (image tower).

\subsection{Dual Encoder Model}

The dual encoder model has one tower that represents the text input which is represented as a bag of words and an embedding generated and the other tower is for he image which is represented as an embedding that is obtained from a ResNet \cite{szegedy2016inception} based model. The dot product similarity of the text and the image embeddings are calculated by the model. In this case, the primary task used to evaluate the model was an image-text retrieval in a zero-shot setting. The models were pretrained with WIT dataset and evaluated on the Flickr30K and MS-COCO test sets. We also trained a model with Conceptual Captions dataset as the pretraining dataset for reference. We used the Recall@1 metric to evaluate the performance of the various models. In this case, for WIT, we used a concatenation of attribution description and reference description and made sure the overall number of tokens was not more than 20. We also filtered the dataset to only English text.

\jc{Should explain what loss function is being used?}

\begin{figure}[ht]
  \centering
  \includegraphics[width=\linewidth]{images/wit_dual_encoder_architecture_diagram.png}
  \caption{WIT Dual Encoder Model for Training.}
  \Description{WIT Dual Encoder Model for Training.}
\end{figure}

\begin{table}
  \caption{Dual Encoder Model: Image-Text Retrieval}
  \label{tab:wit-de-retrieval}
  \begin{tabular}{|l|l|l|l|}
    \hline 
    \textbf{Dataset} 
    & \textbf{R@1 Flickr30K}  
    & \textbf{R@1 MS-COCO}  
    & \textbf{R@1 WIT}\\ 
    \hline 
    \text{CC} 
    & \text{0.103}  
    & \text{0.075}  
    & \text{0.048}\\ 
    \hline 
    \text{WIT} 
    & \text{0.06}  
    & \text{0.042}  
    & \text{0.263}\\ 
  \hline
\end{tabular}
\end{table}


\subsection{Experiments Analysis}

In both these experiments, we found that counter-intuitively that WIT as a pretraining dataset when evaluated in a zero-shot setting did not perform as well as other datasets. Further, we also created a test set out of the WIT data and when we evaluated the models trained on one of the other (non-WIT) datasets, they performed much lower than their usual numbers. This led us to probe into the characteristics especially the ways in which it is different from the other datasets used. 
\jc{Hi Krishina,  I still have some concern on the conclusion you made here: since you are using batch-softmax loss, the better your data is, the worse performance you may get. This is because high-quality text-image pairs means doing batch-softmax (i.e., distinguish a positive item from random negatives) is easy. For this reason, My personal opinion is that the performance on retrieval tasks does not tell us much about the quality of WIT dataset.}

\subsubsection{Language Representation}

The first thing we noticed is that the test sets are all English based whereas roughly only about 50\% of the data in WIT is in English. So we used only English text for the rest of the experiments.

\subsubsection{Vocabulary Analysis}

Next, we analyzed the vocabulary of WIT dataset. Since Wikipedia is very entity heavy and is a wide and deep knowledge base, our suspicions were confirmed that WIT dataset and hence its vocabulary is very diverse. For example, we found that over 72\% of the unigrams from the text descriptions (just the reference description) occur 3 times or less.

\begin{table}[h]
  \caption{Vocabulary Comparison}
  \label{tab:wit-vocab}
  \begin{tabular}{|l|r|r|r|}
    \hline 
    \textbf{Dataset} 
    & \textbf{Unigrams}
    & \textbf{freq <= 3}
    & \textbf{pct freq <= 3}\\ 
    \hline 
    \text{CC} 
    & \text{149,924}
    & \text{63,800}
    & \text{42.55\%}\\  
    \hline 
    \text{WIT} 
    & \text{867,906}
    & \text{625,100}
    & \text{72.02\%}\\  
  \hline
\end{tabular}
\end{table}

\subsubsection{Language Model}

We further looked at the unigram distribution as a Language Model representation and used Jensen-Shannon Divergence to compare it against the various other datasets including the test sets. This too shows that WIT vocabulary and language model is not as similar to the test sets such as Flickr 30K and MS-COCO.

\begin{table}
  \caption{Language Model Comparison}
  \label{tab:wit-lang-model}
  \begin{tabular}{|l|p{.30\linewidth}|}
    \hline 
    \textbf{Dataset A vs B} 
    & \textbf{Jensen-Shannon Divergence}\\ 
    \hline 
    \text{Flickr vs Flickr Test}
    & \text{0.1679}\\  
    \hline 
    \text{COCO vs COCO Test}
    & \text{0.1008}\\  
    \hline 
    \text{CC vs Flickr Test}
    & \text{0.4844}\\  
    \hline 
    \text{CC vs COCO Test}
    & \text{0.4746}\\  
    \hline 
    \text{CC vs WIT}
    & \text{0.3825}\\  
    \hline 
    \text{WIT vs Flickr Test}
    & \text{0.6007}\\  
    \hline 
    \text{WIT vs COCO Test}
    & \text{0.5957}\\  
  \hline
\end{tabular}
\end{table}

% entity comparison
% text caption size comparison
% image size comparison

\subsubsection{Entities Analysis}

We also used an existing image classification model to tag all the WIT images with entity classes. We once again found that a large number (over 80\%) of the entities occur 3 times or less. This posts another unique challenge to machine learning models that the examples are all unique in many ways and even though there is plenty of data, there is not much repetition of the same thing.


\subsection{Effectiveness of Various Text Fields}

For the same image-text retrieval experiment, we performed different variations using different text fields or a combination of them.

We find that very long texts do not help these model for a retrieval task. Also given that it is a bag of words model for the text tower, we believe that might be further exacerbating the confusion in learning. Of all the text combinations, just using reference description and attribution description by itself and kept to a short length shows the best performance. There might be other tasks or models that could benefit from a shorter text (e.g. Page Title or an Entity) or a general form of longer text (e.g. Page Description which is about a few sentences long and is about the whole page) or a specific form of longer text (e.g. Section Text which is a few sentences from the section in which the image existed) or even different combinations (e.g. concatenations) of these texts as they see fit. Reference Description and Attribution Description are the two fields that come closet to an almost single line text caption that we generally associate with image-text example pairs.

\begin{table}[]
\caption{Dual Encoder Model with Retrieval Task}
\label{tab:wit-de-exp-retrieval}
\begin{tabular}{|c|c|c|c|}
\hline
\multirow{2}{*}{Text} & \multicolumn{3}{c|}{Recall@1} \\ \cline{2-4} 
                  & Flickr30K & MS-COCO & WIT \\ \hline
  \text{attr + page}
    & \text{0.045}
    & \text{0.033}
    & \text{0.289}\\
    \hline
    \text{attr + title}
    & \text{0.053}
    & \text{0.033}
    & \text{0.255}\\
    \hline
    \text{ref + page}
    & \text{0.043}
    & \text{0.031}
    & \text{0.266}\\
    \hline
    \text{ref + title}
    & \text{0.05}
    & \text{0.041}
    & \text{0.217}\\
    \hline
    \text{attr (len20)}
    & \text{0.05}
    & \text{0.034}
    & \text{0.234}\\
    \hline
    \text{attr (len 40)}
    & \text{0.042}
    & \text{0.027}
    & \text{0.221}\\
    \hline
    \text{ref (len20)}
    & \text{0.04}
    & \text{0.033}
    & \text{0.175}\\
    \hline
    \text{ref (len 40)}
    & \text{0.032}
    & \text{0.025}
    & \text{0.142}\\
    \hline
    \text{ref + attr (len 20)}
    & \text{0.06}
    & \text{0.042}
    & \text{0.263}\\
  \hline
\end{tabular}
\end{table}

\subsection{WIT is Different}

Thus, we arrive at a conclusion that WIT is a very different dataset than the existing datasets. For one, WIT is immensely useful given that it is based off of Wikipedia and it represents real world knowledge that has been constructed over nearly two decades. Next, the quality of the dataset has been maintained by many filtering rules we have implemented and further analyzed and confirmed via random sampling and ratings. Given that WIT represents over 100 languages, it is a huge plus but there are no current test datasets to simply evaluate it against. We hope that WIT will be the first of its kind for dozens of languages. Also, we find that WIT is very rich and diverse in entities, vocabulary and language model and this should only help models learn more about the real world.

